SwarMer: A Decentralized Localization Framework for Flying Light Specks

Swarm-Merging, SwarMer, is a decentralized framework to localize Flying Light Specks (FLSs) to render 2D and 3D shapes. An FLS is a miniature sized drone equipped with one or more light sources to generate different colors and textures with adjustable brightness. It is battery powered, network enabled with storage and processing capability to implement a decentralized algorithm such as SwarMer. An FLS is unable to render a shape by itself. SwarMer uses the inter-FLS relationship effect of its organizational framework to compensate for the simplicity of each individual FLS, enabling a swarm of cooperating FLSs to render complex shapes. SwarMer is resilient to both FLSs failing and FLSs leaving to charge their battery. It is fast, highly accurate, and scales to remain effective when a shape consists of a large number of FLSs.

==> arch.tex <==
A 3D FLS display consists of a number of software and hardware components.  These include hangers that protect FLSs from external factors that may either damage them or reduce their lifetime.  A hanger may be accessible to one or more Dispatchers, Charging Stations, and Terminus.

Charging Stations charge the battery of FLSs, depositing those with a fully charged battery to a hanger.  A charging station has one or more well defined entry points known to the FLSs.  

Dispatchers deploy FLSs to render an illumination.  One or more hangers may be accessible to a dispatcher.  Dispatchers may communicate identity, flight path, and deploy time of their FLSs to one another to detect potential FLS crashes.  %Each dispatcher has a unique id.  This id is used to implement a decentralized algorithm to avoid potential crashes, see Section~\ref{sec:static}.

Garbage Collectors, GCs, collect failed FLSs that fall to the bottom of the display and bring them to a Terminus.  A GC may be in the form of a conveyor belt that moves failed FLSs away from the display grid and into entry points that open to the Terminus.

A Terminus has one or more entry points in the display.  In addition to GCs, an FLS that detects it may no longer function properly may fly to a Terminus, see Section~\ref{sec:failure}.  %A Terminus may diagnose a failed FLS, perform procedures to recover it to normal mode of operation, and deposit a recovered FLS to a hanger. 

An Orchestrator is a software component that manages FLSs in Hangers, Charging stations, Dispatchers, Garbage Collectors, and Terminus.  It also manages the storage and network of the Hub.  The Orchestrator may delegate tasks to other components.  %For example, it may delegate deployment of FLSs to one or more dispatchers.%, see Section~\ref{sec:static}.  

Finally, a Hub provides the processing, storage, and networking capabilities of the FLS display.  It uses an off-the-shelf operating system.  The Hub executes the Orchestrator software.% that manages and coordinates all aforementioned components.


The Orchestrator implements centralized algorithms to render a motion illumination.  It may also implement hybrid centralized and decentralized algorithms that include the participation of the FLSs.  For example, with the reliability technique of Section~\ref{sec:failure}, the Orchestrator may identify the number of FLSs in a group and their identity.  However, detection of FLS failures and subsequent substitution of a standby FLS for the failed FLS is performed by the FLSs without the Orchestrator involvement.  Certain tasks may be implemented in a decentralized manner independent of the Orchestrator, e.g., collision avoidance implemented by FLSs.

==> discuss.tex <==

This section discusses diverse topics related to the design of SwarMer and its rendering of shapes.


\begin{figure}
\centering
\includegraphics[width=3.5in]{figs/randomPlacement.jpg}\hfill
\caption{Random placement.}
\label{fig:randomPlacement}
\end{figure}

\subsection{Random FLS placement}\label{sec:random} 
SwarMer will work with a random placement of FLSs in a 3D display as long as the coordinates of a point are assigned to each FLS.
A limitation is that the shape may be shifted along the different axes by a wide margin because SwarMer is a relative localization technique.
The precise amount of shift depends on how FLSs form swarms, and how swarms merge and move.  
To illustrate, consider the 3D dragon of Figure~\ref{fig:diff3D}.
We assign FLSs to a 3D space using a random number generator, see Figure~\ref{fig:randomPlacement}.a.
FLSs use SwarMer to localize and render the dragon with a Hausdorff distance less than 0.09 in 26 rounds, see Figure~\ref{fig:randomPlacement}.b.
The dragon is shifted along the different axes.
One may address this limitation by having one {\em oracle} FLS configured with specialized hardware that computes its position with a high accuracy, extending SwarMer as follows.
First, a swarm that localizes relative to the oracle inherits its oracle property. 
A swarm with the oracle property does not localize relative to other swarms.
All other swarms are required to localize relative to it and inherit its oracle property.
This prevents shifting of the shape across different axes.

%\subsection{Impact of error}\label{sec:error}
%Hence, an implementation of SwarMer should strive to enhance the accuracy of the angle of the localizing FLS relative to its anchor, improving the quality of shapes.

%The quality of SwarMer renderings and their Hausdorff distance is impacted by the error in the angle of the localizing FLS relative to its anchor FLS and the error in the dead reckoning of the localizing FLS.
%Our experiments show SwarMer is more sensitive to the error in the angle of the localizing FLS to its anchor.
%Minimizing this error improves SwarMer's quality of renderings.

%An implementation of SwarMer may suffer from packet loss.  This may cause some FLSs in a swarm to not receive the message that contains either change of status or vector of movement.
%Both are important and constitute our future research direction.
%\noindent{\bf Impact of error:}
%Errors such as %lost messages that prevent SwarMer from constructing a single swarm for a shape may impact its accuracy.
%In general,
%Lost packets may 
%This impact either the quality of an illumination (Hausdorff distance), the time (rounds) required to render an illumination, or both.

%We emulated packet loss by introducing the following simple error in our simulator.  At the end of each round, an FLS leaves its swarm with a fixed probability $q$ by changing its Swarm-ID to its FID.  This error impacted alternative shapes differently.  With the dragon and a small value of $q=0.00075$, we were pleasantly surprised to observe the number of rounds required to achieve an HD lower than 0.09 was lowered to 17 from 22.  This trend continued as we increased $q$ to $0.001$ with the number of rounds reduced to 15.  However, the number of rounds jumps to 58 with $q=0.005$ and 168 with $q=0.01$. With $q \geq 0.1$, we terminated the experiment at 500 rounds because SwarMer did not construct a single swarm and its Hausdorff distance (0.53 with $q=0.1$) did not drop below 0.09. Multiple swarms were visible with $q=0.5$ at round 500.  See Figure~\ref{fig:multipleswarms}.
%\centering
%\includegraphics[width=3.5in]{figs/dragonMultipleSwarms.jpg}\hfill
%\caption{FLSs part from their swarms with 0.5 probability.}
%\label{fig:multipleswarms}
%\end{figure}


%With $q \geq 0.1$, the introduced error produced many individual FLSs at the end of a round.  Some cause different swarms to localize relative to them instead of one another. This prevents swarms to merge into one.  Disjoint swarms diminish the quality of a rendering, producing fragmented shapes. Swarms are required to localize and become one to render a shape accurately.



%\subsection{Swarm With Many Anchor FLSs and One Localizing FLS}\label{sec:Manchor1localizing}
%A swarm may have at most one localizing FLS and many anchor FLSs at the same time.  Figure~\ref{fig:multipleswarms} shows the number of such occurrences with 3D shapes of Figure~\ref{fig:cmp3D} in different rounds.

%\begin{figure}
%\centering
%\includegraphics[width=3.5in]{figs/fig30-Number of swarms merged into a busy swarm.jpg}\hfill
%\caption{Number of times a swarm merged into a busy swarm with at most one localizing FLS.}
%\label{fig:multipleswarms}
%\end{figure}

==> failure.tex <==
An FLS is a mechanical device that may fail.  Its failure may reduce the quality of an illumination by not rendering its points.
There are several types of FLS failures:
rotor failures,
light source failures, 
computing failures in the form of reboots,
and battery power failures.
Assuming these failures are independent and occur at a constant rate, one may compute the Mean Time To Failure of an FLS ($MTTF$) similar to how magnetic disk manufacturers calculate the MTTF of disk drives~\cite{gibson}.
The Mean Time to Degraded Illumination (MTDI) is a linear function of the number of FLSs ($\alpha$) that constitute an illumination:  $MTDI=\frac{MTTF~of~1~FLS}{\alpha}$.

%A failed FLS results in loss of its assigned lightings and flight paths, degrading the quality of an illumination.  The Mean Time to Degraded Illumination (MTDI) is a linear function of the number of FLSs ($\alpha$) that constitute an illumination:  $MTDI=\frac{MTTF~of~1~FLS}{\alpha}$. 

Assuming an FLS fails once a month (MTTF of 720 hours), the MTDI of the Rose illumination with $\alpha$=65,321 FLSs is 40 seconds.
This is disheartening if we want to scale to illuminations consisting of millions of FLSs.
Below, we describe a technique to enhance MTDI of an illumination in the presence of frequent FLS failures.  We start by describing how FLSs cooperate to detect failures.  Subsequently, we describe the use of standby FLSs, and data replication and parity techniques to improve MTDI.

FLSs cooperate to detect failures and notify the Orchestrator of the identity of the failed FLS.
This cooperation is in two forms.
First, once an FLS detects its own failure, it communicates this information with its neighbors and the Hub (Orchestrator) using its networking capability. This applies to the first two forms of failures.  
%With light source failures, the FLS flies to a Terminus immediately as it is no longer able to display an illumination.
%With rotor failures, it repels~\cite{roguedrone2021,repel1,repel2} FLSs in its downward descent by generating frequent failed messages.  Those FLSs that receive this message move away to prevent the failed FLS from crashing into them.    

Second, FLSs exchange periodic heartbeat messages~\cite{can2001,chord2001} with their neighbors in the display mesh to detect processor and battery failures.
An FLS that encounters these forms of failures may not able to notify other FLSs of its failure.
Hence, FLSs detect such failed FLSs using periodic messages.  
%This is because an FLS that encounters such failures 
%The last two forms of failures prevent an FLS from notifying other FLSs.  
%The detection mechanism requires FLSs to exchange periodic heartbeat messages with their neighbors in the display mesh.  
If an FLS does not receive an anticipated heart beat message from one of its neighbors then it polls that neighbor.
After a few failed attempts, it identifies the neighbor as having failed and communicates the identity of this failed FLS to other neighbors.
This information propagates throughout the FLS swarm and the display Hub to the Orchestrator.  

To maintain the quality of illumination, a failed FLS must be replaced with a new one instantaneously.
We realize this by deploying standby FLSs.
In normal mode, standby FLSs are dark.  After the discovery of a failed FLS, the standby occupies the display cell of the failed FLS and assumes its lighting responsibility to render the illumination.
This occurs concurrently with the Orchestrator deploying a replacement FLS to substitute for the standby.

More formally, $G$ FLSs neighboring one another in the display mesh form a group with one standby FLS.
The minimum value of $G$ is one, requiring
a standby for every FLS that is rendering a point.
This standby mirrors the flight paths assigned to its paired FLS.
If an FLS fails, its standby resumes its lighting and flight responsibilities immediately.  
A challenge of $G$=1 is how to prevent the standbys from obstructing the user's field of view (FoV).

With $G>1$, if the standby FLS has sufficient storage then it may maintain a copy of the flight paths assigned to the $G$ FLSs.  Otherwise, it may compute the parity of the $G$ flight paths using xor of the bits.% representing flight paths assigned to the $G$ FLSs.
The resulting parity data is the same size as the flight data assigned to an FLS in the group.

Parity techniques are more space efficient than replication techniques.
However, to compute the missing flight path of a failed FLS in the group, they require the standby to obtain and use the flight paths of the remaining $G-1$ FLSs.
Using this data in combination with its parity data, the standby computes the flight paths and illumination responsibilities of the failed FLS.  
With more than 1 failure in a group, the standby must wait for the Orchestrator dispatched FLSs to arrive with their flight data before the standby is able to compute the missing flight path.

A large value of $G$ increases the probability of two or more FLSs failing in a group simultaneously.
With replication, the standby may substitute for one failed FLS.  The illumination quality may suffer until the Orchestrator's dispatched replacements arrive and substitute for the other failed FLSs. 

%\subsection{Group Construction}
The $G$ FLSs that participate in a group must be in close proximity of one another.  This minimizes the distance travelled by a standby to substitute for a failed FLS.  If the group is using a parity scheme, close proximity also provides for local communication between the standby and the remaining $G-1$ FLSs to compute the flight path and lighting responsibilities of the failed FLS. 

FLS group construction is a weighted matching problem~\cite{tutte47,edmonds65}.
There exists centralized~\cite{avis83,preis99}, distributed~\cite{hoepman2004}, and decentralized~\cite{kclique2014} algorithms for this problem.
With static illuminations, one may adapt these for use by the Orchestrator, multiple dispatchers, and millions of FLSs, respectively.
See~\cite{anon2}.%This is a short-term future research direction.

With motion illuminations, the position of some FLSs will change from one point cloud to the next.  This may change the distance between FLSs that constitute a group.
The FLSs may re-construct the groups using decentralized~\cite{kclique2014} algorithm.
Other alternatives are detailed in~\cite{anon2} and eliminated due to space constraints.
%This may require re-assignment of standbys.  With a parity technique, an impacted standby must re-compute its parity information for the new group. The system may relax the value of $G$ for evolving groups, allowing some groups to consist of more than $G$ FLSs and others to consist of fewer than $G$ FLSs.    

%Another approach is to maintain the same FLS membership for the group and require the standby to adjust its position to have approximately the same distance to the different FLSs that constitute the group.  If the FLS reliability is heterogeneous, the standby may position itself closer to those FLSs with a higher failure probability.  

%Yet another possibility is to remove the constraint that each FLS must belong to a group.  This enables an FLS to leave a group and possibly join another group, requiring the standby of the impacted groups to adjust its membership information and replicated/parity data.  An FLS crucial to the illumination may have a mirror standby.  

%An investigation of these possibilities is a future research direction.    

%\subsection{MTDI using Groups}:
In~\cite{anon2}, we present models 
to establish the MTDI of an illumination as a function of $G$.  Due to lack of space, we present only the results obtained from these models.  Table~\ref{tbl:parity} shows MTDI of the Rose illumination assuming an FLS fails once a month and the display's MTTR is 1 second.
The reliability groups enhance MTDI from 40 seconds to almost two months with 20 FLSs in a group, $G$=20.
This is enhanced almost two folds (to 111 days) with 10 FLSs per parity group, $G$=10.
With $G$=10, the Rose illumination requires approximately 6,400 additional FLSs, a 10\% overhead. 

\begin{table}
\begin{small}
  \caption{Reliability groups enhance MTDI.}
  \label{tbl:parity}
  \begin{tabular}{c|cc}
    \toprule
    & G=10 & G=20\\
    \midrule
    Total Number of FLSs & 71,853 (1.1$\alpha$) & 68,588 (1.05$\alpha$) \\
    Overhead Cost & 10\% & 5\% \\
    MTDI (Hours) & 2670 & 1399 \\
    %$\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{small}
\end{table}

 



==> future.tex <==
Localization of FLSs to render shapes is a novel topic with many exciting short term and long term research directions.
A short term objective is to develop a communication protocol that facilitates message passing among FLSs to implement SwarMer.
Such a protocol may encompass various features, including the ability to modify the state of other FLSs, determine the membership of an FLS in a swarm, estimate the size of a swarm, determine communication range, and optimize bandwidth utilization, among others.
It provides insight into the different kinds of errors that may occur.
Section~\ref{sec:error} highlighted the importance of constructing one swarm and how an error that prevents one swarm will diminish the quality of a rendering.
A key research question is what are the other qualitative errors?  What factors such as race conditions contribute to them?  And, how can the impact of these errors be minimized?
%These can be studied and addressed in the context of a robust communication protocol.
Once a robust protocol is developed, we intend to use it to implement SwarMer in a testbed consisting of 50 Crazyflies localized using Vicon.
Vicon is a highly accurate centralized localization system as described in Section~\ref{sec:related}.
The testbed provides a comparison of SwarMer with the Vicon, quantifying their tradeoffs.

A long term objective is to extend SwarMer to support motion illuminations and FLS-matter~\cite{shahram2021,shahram2022}.
A motion illumination consists of a sequence of point clouds rendered as a function of time.
FLS-matter requires an FLS to detect the force exerted against it by measuring the degree of its displacement and the amount of time required for this displacement.
SwarMer may be extended to support both use cases.

==> stag.tex <==
STAG is a novel algorithm that staggers charging of FLS batteries as a function of time with the objective to minimize both the number of charging stations and the overall number of FLSs to render an illumination.  STAG has an initial startup overhead.  This overhead is in the form of either a higher latency when rendering an illumination or wasted energy.
Due to space limitations, we refer the interested reader to~\cite{anon2} for this detail.
%We quantify this overhead and show STAG may trade one for the other at the end of this section.

STAG makes several assumptions.  First, each FLS has a battery that provides a finite flight time $\beta$ when fully charged.  Second, $\Omega$ time units are required to fully charge a depleted battery with minimal or no remaining flight time left.  %Third, the time to charge an FLS battery, $\lambda$, is a linear function of $\beta$ and its remaining flight time $r$, $\lambda$=$\frac{\Omega*r}{\beta}$.  
%Fourth, STAG assumes a parity based technique using standby FLSs is used to tolerate FLS failures.  The battery of these standbys is similar to the other FLSs.  

An FLS computes the amount of battery flight time to fly to a charging station using its distance to the charging station.  Once its battery flight time reaches this threshold, the FLS will go dark and fly to the charging station.

A standby FLS (see Section~\ref{sec:failure}) will substitute for this FLS to perform its lighting responsibility while a dispatcher will deploy an FLS with $\beta$ flight time to substitute for the standby.  %%The FLS flying back may be the standby for the group.  

It is important to minimize the window of time $\Delta$ for a battery depleted FLS$_d$ to switch places with a fully charged FLS$_c$.
Should an FLS belonging to the reliability group of FLS$_d$ fail during $\Delta$, this results in a light/FLS missing from the illumination.  %We address this in Section~\ref{sec:STAGdiscuss}

%{\em Preliminaries:}  Consider an illumination with $\alpha$ FLSs and assume the time to charge the battery of each FLS equals its flight time on a fully charged battery, $\Omega=\beta$.
%A naive algorithm may deploy all $\alpha$ FLSs at one instance in time.  After $\beta$ time units, all FLSs must fly back to a charging station while the dispatchers deploy $\alpha$ fully charged FLSs.  Naive repeats this process every $\beta$ time units while rendering the illumination. 
  
%Naive has several limitations.  First, it requires 2$\alpha$ FLSs to render an illumination:  $\alpha$ FLSs charge while $\alpha$ FLSs render the illumination.  Second, there is an exchange step when fully changed FLSs and fully depleted FLSs switch places.  The illumination may become distorted during this period because almost all FLSs that constitute an illumination may go dark in order to switch places with fully charged FLSs.  Moreover, the algorithm that manages FLSs during this period has a high complexity as it must manage flight patterns of 2$\alpha$ FLSs. 

{\em \bf STAG} staggers FLSs as a function of time to prevent them from exhausting their finite flight time at the same time.  It overlaps charging of some FLSs with others that are rendering an illumination.
%, eliminating Naive's exchange step.  
In its steady state, STAG switches a fully charged FLSs with a fully depleted FLSs continuously.  Details of STAG are as follows.

STAG constructs $h$ flocks of FLSs.  A flock $i$ consists of $\alpha_i$ FLSs.  Within a flock $i$, STAG staggers its $\alpha_i$ FLSs such that their remaining battery flight time ranges from $\beta$ down to the staggering interval S=$ \frac{\beta}{\alpha_i}$.  %More formally, assuming the FLSs in a flock are numbered from 1 to $\alpha_i$, the remaining flight time of FLS $j$ is $\beta(j)=\frac{j*\beta}{\alpha_i}$.  Thus, FLS $j=\alpha_i$ has a fully charged battery with $\beta$ flight time. 

The staggering time interval S is the minimum flight time required by an FLS to travel to a charging station.  The number of FLSs charging (or staged in a hanger) to substitute for an FLS of Flock $i$ FLS is $\lceil \frac{\Omega}{S} \rceil$.  This is the extra number of FLSs required by a flock to render an illumination.  The total number of FLSs that are charging (or staged in a hanger) is $h \times \lceil \frac{\Omega}{S} \rceil$.  There is a startup overhead associated with STAG that we describe in~\cite{anon2}. 

STAG minimizes the number of additional FLSs required to render an illumination.
Its formal theorem and proof are presented in~\cite{anon2}.

The number of FLSs in transit from a charging station to an illumination is $2h$.
With $h=1$, there are 2 FLSs in transit.  One flying from the illumination to a charging station and a second from a charging station to the illumination.
A display must ensure these FLSs are not in the user's field of view.

Given a swarm, reducing its number of flocks to one, $h$=1, minimizes the number of FLSs in transit.  This reduces the likelihood of an in-transit FLS obstructing the user's field of view.  

However, the number of flocks is dictated by the time required for an FLS to fly back to the charging station ($S_{threshold}$) and the number of FLSs required by an illumination $\alpha$.  With an illumination that consists of a large number of FLSs, maintaining $h$ at one results in a small staggering interval S (because S is a function of the number of FLSs in a flock).  
Its lower bound is 
%the flight time (i.e., remaining battery life) required for an FLS to travel to a charging station, 
$S_{threshold}$.  This dictates the number of FLSs in a flock ($\alpha_i=\frac{\beta}{S_{threshold}}$) which in turns dictates the number of flocks, $h=\lceil \frac{\alpha}{\alpha_i} \rceil$.  

%\subsection{Flock Formation} 
\noindent{\em Flock Formation.}
With STAG, flocks are logical.  Unlike the failure handling groups, there is no constraint on them to be in close proximity of one another.
However, similar to forming groups, this matching problem has well known
centralized~\cite{avis83,preis99}, distributed~\cite{hoepman2004}, and decentralized~\cite{kclique2014} algorithms.
An FLS display may adapt one of these techniques to form STAG's flocks, see~\cite{anon2}.
%FLSs may implement and execute such a protocol to form flocks and implement STAG.

%A centralized technique for formation of cliques may require the Orchastrator to compute the number of flocks and the quota for each flock, i.e., the number of FLSs for each flock.  It assigns flock ids to different dispatchers that deploy FLSs.  The dispatchers assign flock ids to their deployed FLSs until the quota for a given flock id is exhausted.

%{\em Startup overhead:}
%STAG must stagger the battery lifetime of FLSs in a flock when an illumination is first initiated.  One approach is to deploy FLSs of a flock every $S$ time units.  The limitation of this approach is that it introduces a delay of $\alpha_i \times S$ time units before the illumination is rendered, its latency.  With large values of $\alpha_i$ and $S$, this latency may be substantial.  For example, with the 65321 FLSs required by the Rose illumination, assuming $S$ is 100 milliseconds, the startup latency to render the illumination is more than 10 minutes.  

%Alternatively, STAG may waste energy by requiring dispatchers to deploy FLSs with full batteries as fast as possible and require FLSs with partially full batteries to fly back to be recharged.  To illustrate, with Example 1, relative to time T when all 5 FLSs are deployed, FLS 1 flies back after T+3 minutes to fully charge its battery while FLS 6 flies to substitute for FLS 1.  FLS 2 flies back after T+6 minutes to fully charge its battery while FLS 1 flies to substitute for FLS 2.  FLS 3 flies back after T+9 minutes to fully charge its battery while FLS 2 flies to substitute for FLS 3.  Note that FLS 1 and 2 have partial flight time left and are staggered in time. 

%The ordering is dictated by the ID of the FLSs and may be implemented in a decentralized manner.  When FLS 1 flys back, the extra FLS flies to substitute for it and assume its ID.  When the 2nd FLS flys back, the 1st FLS is fully charged and substitutes for it.  This continues a few more iterations until it reaches a steady state.  In this state, the remaining flight time of an FLS$_j$ is almost fully exhausted before it flies back to the charging station and a fully charged FLS is deployed to substitute in FLS$_e$'s vacant cell (or the cell occupied by its standby). 

%The alternative wastes energy because it requires FLSs with partially charged batteries to fly to a charging station to become fully charged.  Thus, the tradeoff between the two techniques is startup latency versus wasted energy.  A hybrid of the two is possible where a technique specifies an upper bound on either the amount of energy or the tolerable startup latency.

 
\begin{table}
\begin{small}
  \caption{STAG with different $\beta$ and $\Omega$ values.}
  \label{tbl:stag}
  \begin{tabular}{l|ccc}
    \toprule
    & $\beta$=5 min & $\beta$=10 min & $\beta$=20 min \\
     & $\Omega$=10 min & $\Omega$=5 min & $\Omega$=2.5 min \\
    \midrule
    $h$, number of flocks & 218 & 109 & 55 \\
    $\alpha_i$, FLSs/Flock & 300	& 600 & 1200 \\
    Extra FLSs per Flock & 600 & 300 & 150 \\
    \midrule
    FLSs for the last Flock & 221 & 521 & 521 \\
    S for the last flock (Millisec) & 1358 & 1152 & 2303 \\
    Extra FLSs for the last flock &	442 & 261 & 65.125 \\
    \midrule
    Extra FLSs for the illumination & 130642 & 32661	& 8166 \\
    Overhead Cost & 200\% & 50\% & 12.5\% \\
    Total Number of FLSs & 195,963 & 97,982 & 73,487 \\
    %$\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{small}
\end{table}

%\subsection{An Analysis}
\noindent{\em An Analysis.}
Table~\ref{tbl:stag} quantifies the behavior of STAG with different $\beta$ and $\Omega$ values.  The first column pertains to the flight time and battery charge time of today's Sky Viper Dash Nano Drone (\$17).  
The other two columns correspond to anticipated future generations of this drone with flight time on a fully charged battery ($\beta$) doubling and the time to charge ($\Omega$) its battery halving. 

We set $S_{threshold}$ to 1 second.
It defines the number of FLSs in a flock, $\alpha_i$, shown in the 2nd row of Table~\ref{tbl:stag}.  The number of FLSs that constitute the Rose illumination ($\alpha$=65,321) is not an even multiple of $\alpha_i$.  Hence, the middle 3 rows show the characteristics of the last flock that has the remaining FLSs.  Its value of $S$ is higher than 1 second (1000 millisec) because it has fewer FLSs.  

The characteristics of today's Sky Viper battery increases the number of FLSs to render the Rose illumination 3 folds.  This is a 200\% overhead.  This overhead decreases linearly as we enhance battery characteristics,
see the 2nd to last row of Table~\ref{tbl:stag}.
With an 8 fold overall improvement in battery characteristics (4 fold enhancement of $\beta$ and 4 fold reduction of $\Omega$), STAG's overhead decreases to 12.5\%.   

